S2R-DepthNet: Learning a Generalizable Depth-specific Structural Representation

Human can infer the 3D geometry of a scene from a sketch instead of a realistic image, which indicates that the spatial structure plays a fundamental role in understanding the depth of scenes. We are the first to explore the learning of a depth-specific structural representation, which captures the essential feature for depth estimation and ignores irrelevant style information. Our S2R-DepthNet (Synthetic to Real DepthNet) can be well generalized to unseen real-world data directly even though it is only trained on synthetic data. S2R-DepthNet consists of: a) a Structure Extraction (STE) module which extracts a domaininvariant structural representation from an image by disentangling the image into domain-invariant structure and domain-specific style components, b) a Depth-specific Attention (DSA) module, which learns task-specific knowledge to suppress depth-irrelevant structures for better depth estimation and generalization, and c) a depth prediction module (DP) to predict depth from the depth-specific representation. Without access of any real-world images, our method even outperforms the state-of-the-art unsupervised domain adaptation methods which use real-world images of the target domain for training. In addition, when using a small amount of labeled real-world data, we achieve the state-ofthe-art performance under the semi-supervised setting. The code and trained models are available at https://github.com/microsoft/S2R-DepthNet.

==> backup.tex <==
%In order to effectively extract structural information from images, we propose a Structure Extraction Network (SE-Net), which is shown in Figure \ref{fig:overview}. Our proposed Structure Extraction Network includes an encoder part $E_{struct}$ and a decoder part $D_{struct}$. The encoder is used to encode the structure information of the input image, discarding redundant style information, and the decoder is used to decode the encoded structure information into structure map.  

% Inspired by previous work  
% Because we also need to disentangle structure and style,  we utilize Huang \etal\cite{huang2018munit}'s methods to generate encoder of our Structure Extraction Network $E_{s}$. However, because our tasks are different, we modified the original methods of Hu \etal \cite{huang2018munit} to suit depth estimation task.
% Next, I will introduce the the encoder $E_{struct}$ of Structure Extraction Network we proposed in detail, and focus on the difference between our method and \etal\cite{huang2018munit}'s method. 

% As shown in Figure \ref{fig:SE-Net}, given a source-domain image $x^s$ as input, the shared structure encoder $E_{struct}$ produces $c_{struct}^{s} = E_{struct}(x^s; \theta_{struct})$ to present its domain-invariant structure information while the source-specific private style encoder $E_{style}^{s}$ generates $c_{style}^{s} = E_{style}^{s}(x^s; \theta_{style}^{s})$ for capture its remnant aspects that are largely related to domain-specific, low-level texture information. These two components ${c_{struct}^{s}, c_{style}^{s}}$ are complementary to each other. Combining these two codes, the original image can be restored by decoder $\mathcal D_{s}$. Since in our settings, it is impossible to obtain images of target domain and the style of real images of target domain cannot be obtained. Therefore, we hope that the structure encoder $E_{struct}$ can be insensitive to any style of images. 

% Inspired by previous work\cite{geirhos2018,jackson2019style}, Geirhos \etal \cite{geirhos2018} show that ImageNet-trained CNNs are strongly biased towards recognising textures rather than shapes, because the CNNs tends to learn texture features  that are easier to learn, which could be seen as a version of Occam's razor. Jackson \etal \cite{jackson2019style} claim CNNs are easy to overfit due to  texture features, so they proposed a Style augmentation using style transfer to augment the original data to learn style-irrelevant features for avoiding overfitting. 

% Therefore, in order to enable our structural encoder to extract structural features that are not sensitive to any kind of style, we use a common style dataset "Kaggle Painter By Numbers (PBN)" dataset, consisting of a large of paintings across many genres as another branch of the network.
% By sharing the structure encoder $E_{struct}$, the encoder can see various styles of data and extract structural features that are not sensitive to styles.
% Similar to the operation mentioned above, painter images $x^p$ can also be decomposed into code $c_{struct}^p$ representing structure and code $c_{style}^p$ representing style. Formally, $c_{stuct}^p = E_{struct}(x^p; \theta_{struct})$ and $c_{style}^p=E_{style}^p(x^p; \theta_{style}^p)$. These two codes can also restore the original  painter images through a decoder $\mathcal D_{p}$.


% \begin{figure*}[htp]
% 	\centering
% 	\includegraphics[width=0.9\textwidth]{figs/SE-Net.pdf}
% 	\caption{ Our structure encoder of Structure Extraction Network (SE-Net) training framework. The training framework consists a shared structure encoder $E_{struct}$ which  is used to extract domain-invariant structural features, two specific private style encoder $E_{style}^{s}$ and $E_{style}^{p}$, which extract domain-specific style features of  each image, two unique decoder $D_s$ and $D_p$, which are used to reconstruct original image and translated images for calculating  the loss.} 
% 	\label{fig:SE-Net}
% \end{figure*}

% Then we will combine the $c_{struct}^{s}$ extracted from the source domain data with randomly draw a style latent code $c_{style}^{p}$ from the prior distribution $q(c_{style}^{p}) \sim \mathcal N(0, I).$  
% We use $\mathcal D_{p}$ to produce the final output image $x_{s\to p} = \mathcal D_{p}(c_{struct}^s, c_{style}^{p})$. 
% Similarly, we will also combine the $c_{struct}^{p}$ extracted from the painter images with randomly draw a style latent code $c_{style}^{s}$ from the prior distribution $q(c_{style}^s) \sim \mathcal N(0, I)$. 
% We will use $\mathcal D_{s}$ to produce the final output image $x_{p\to s} = 
% \mathcal D_{s}(c_{struct}^p, c_{style}^s)$.

% In order to effectively disentangle the structure code and the style code from the original image. 
% The training of the entire structure code extractor requires the following loss.
% \paragraph {Image reconstruction loss.} Given an image sampled from the data distribution, because the two parts are complementary, so we can decode them back to the original image.
% \begin{align}
% \begin{autobreak}
% \mathcal  L_{recon}^{x_s} = \mathbb E_{x_s \sim p(x_s)}[||\mathcal D_s(E_{struct}(x_s), E_{style}^s(x_s)) - x_s||]
% \end{autobreak}
% \end{align}
% \paragraph {Latent reconstruction loss.} 
% After obtaining the final image $x_{s\to p}$ after cross-domain translation, we input it to the shared structure encoder and specific style encoder, so that the obtained latent code can also be reconstructed.
% \begin{align}
% \begin{autobreak}
% \mathcal L_{recon}^{c_{struct}^{s}} = 
% \mathbb E_{c_{struct}^{s} \sim p(c_{struct}^s), c_{style}^p \sim q(c_{style}^p)}
% [||E_{struct}^{p}(\mathcal D_{p}(c_{struct}^s, c_{style}^p)) - c_{struct}^s||]
% \end{autobreak}
% \end{align}

% \begin{align}
% \begin{autobreak}
% \mathcal L_{recon}^{c_{style}^{p}} = 
% \mathbb E_{c_{struct}^{s} \sim p(c_{struct}^s), c_{style}^p \sim q(c_{style}^p)}
% [||E_{style}^{p}(\mathcal D_{p}(c_{struct}^s, c_{style}^p)) - c_{style}^p||] 
% \end{autobreak}
% \end{align}
% where  $q{c_{style}^p}$ is the prior is the prior $N(0, I)$.
% \paragraph{Adversarial loss.} We also use the adversarial loss to match the distribution of the translated images to the painter data distribution. In other words, images generated by our model should be indistinguishable from painter dataset.
% \begin{align}
% \begin{autobreak}
% \mathcal L_{adv}^{x_p} = 
% \mathbb E_{c_{struct}^{s} \sim p(c_{struct}^p), c_{style}^p \sim q(c_{style}^p)}
% [log(1-\mathcal Dis_p(x_{s\to p}))] + 
% \mathbb E_{x_{p}\sim p(x_{p})}[log \mathcal Dis(x_p)]
% \end{autobreak}
% \end{align}

% Where $\mathcal Dis_p$ is a discriminator that tries to distinguish between translated images and painter images. 
% For the another branch, all losses are defined to be similar.
% Through these loss functions, the structure and style of the image can be effectively disentangled.
% Total loss is:
% \begin{align}
% \nonumber \min\limits_{(E,  D_{s}, D_{p}, \mathcal Dis_{s}, \mathcal Dis_{p})} &\max\limits_{(\mathcal Dis_{s}, \mathcal Dis_{p})}  \mathcal L = \\
%  \nonumber&\mathcal L_{adv}^s + \mathcal L_{adv}^p + \lambda_1(L_{recon}^s + L_{recon}^p)+   \\
% &\lambda_2(\mathcal L_{recon}^{c_{style}^{p}} + L_{recon}^{c_{struct}^{s}} + \\
% \nonumber &\lambda_3 (\mathcal L_{recon}^{c_{style}^{s}} + L_{recon}^{c_{struct}^{p}})
% \end{align}
% Where $\lambda_1, \lambda_2, \lambda_3$  are weights each loss term.

==> dataset.tex <==
\subsection{Datasets}\label{sec:datasets}

For experiments, we follow the common protocol adopted by most prior works ~\cite{zheng2018t2net,abarghouei18monocular,Kundu2018adadepth,zhao2019geometry} for domain adaptation of depth estimation. We use synthetic data (vKITTI \cite{Gaidon2016vkitti} or SUNCG\cite{song2016ssc}) with depth annotations as source domain and real data (KITTI \cite{journals/ijrr/GeigerLSU13} or NYU Depth v2 \cite{silberman2012indoor} ) as target domain. In the following section we will introduce these datasets in detail.

 
\paragraph{vKITTI \cite{Gaidon2016vkitti}} is a photo-realistic synthetic dataset, that contains 21260 image-depth paired generated from five different virtual worlds in urban settings imaging and weather conditions. The resolution of this dataset is $375\times1242$. To train our network, 
we follow prior works \cite{zheng2018t2net,zhao2019geometry}, randomly selecting 20760 image-depth paired as our train datasets.  We downsample all the images to $192\times640$ and data augmentation is conducted including random horizontal flipping with a probability of $0.5$, rotation with degrees of $[-5^{\circ}, 5^{\circ}]$, and brightness adjustment.  Because the ground truth of KITTI and vKITTI are significantly different, the maximum depth of the vKITTI dataset is $655.35m$, and the maximum depth value of KITTI is $80m$, so in order to reduce the influence of ground truth differences, the depth value of vKITTI is usually clipped to $80m$\cite{zheng2018t2net,Kundu2018adadepth}.
\paragraph{SUNCG \cite{song2016ssc}} is a indoor synthetic  dataset, rendered with both OpenGL, which contains 45622 3D houses with various room types.
The image size is $480\times640$. Following previous studies\cite{zheng2018t2net},  we chose the camera locations, poses and parameters based on the distribution of real NYU Depth v2 dataset \cite{silberman2012indoor} and retained valid depth maps using the same criteria as Zheng \etal \cite{zheng2018t2net}. A total of 130190 image-depth pairs are used for training, which are downsampled to $192\times256$ during training.
\paragraph{KITTI \cite{journals/ijrr/GeigerLSU13}} is a outdoor real dataset, which is built for various computer vision tasks for autonomous driving. The images and depth maps are captured for outdoor scenes through a LiDAR sensor deployed on a driving vehicle. The original image resolution is $375\times1241$. In order to evaluate on this dataset fairly, we use the Eigen testing set to evaluate\cite{zhou8100183,zheng2018t2net,Kundu2018adadepth,zhao2019geometry} and using median scaling as reported results following previous work \cite{Kundu2018adadepth,zhou8100183} , expect when using real data for semi-supervised training.

\paragraph{NYU Depth v2 \cite{silberman2012indoor}} is real indoor dataset, which contains 464 video sequences of indoor scenes captured with Microsoft Kinect. The dataset is wildly used to evaluate monocular depth estimation tasks for indoor scenes. Following previous work\cite{zheng2018t2net,Kundu2018adadepth,hu2019revisiting,Chen2019structure-aware}, we use the official 654 aligned image-depth pairs for evaluating and use median scaling as reported results\cite{Kundu2018adadepth}.
The size of image is $480\times640$. 
